Task-Specific Skill Localization in Fine-tuned Language Models

Pre-trained language models can be fine-tuned to solve diverse NLP tasks, including in few-shot settings. Thus fine-tuning allows the model to quickly pick up task-specific ``skills,'' but there has been limited study of where these newly-learnt skills reside inside the massive model. This paper introduces the term skill localization for this problem and proposes a solution. Given the downstream task and a model fine-tuned on that task, a simple optimization is used to identify a very small subset of parameters ($\sim0.01$% of model parameters) responsible for ($>95$%) of the model's performance, in the sense that grafting the fine-tuned values for just this tiny subset onto the pre-trained model gives performance almost as well as the fine-tuned model. While reminiscent of recent works on parameter-efficient fine-tuning, the novel aspects here are that: (i) No further re-training is needed on the subset (unlike, say, with lottery tickets). (ii) Notable improvements are seen over vanilla fine-tuning with respect to calibration of predictions in-distribution ($40$-$90$% error reduction) as well as the quality of predictions out-of-distribution (OOD). In models trained on multiple tasks, a stronger notion of skill localization is observed, where the sparse regions corresponding to different tasks are almost disjoint, and their overlap (when it happens) is a proxy for task similarity. Experiments suggest that localization via grafting can assist certain forms of continual learning.

==> Ablation.tex <==
\section{Intersection among the stitches}


\begin{figure}[!tbh]
 \centering
 \begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{Experiments/Progress_Accuracy_model_stitch_4096-shot_test.png}
 \caption{ Model Stitch Accuracy on test set QNLI 4096-shot }
 \label{fig:Progress_Accuracy_model_stitch_4096-shot_test}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{Experiments/Progress_Accuracy_model_stitch_4096-shot_train.png}
 \caption{ Model Stitch Accuracy on train set QNLI 4096-shot }
 \label{fig:Progress_Accuracy_model_stitch_4096-shot_train}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{Experiments/Progress_Accuracy_model_stitch_4096-shot_train_and_test_inter.png}
 \caption{  }
 \label{fig:Progress_Accuracy_model_stitch_4096-shot_train_and_test_inter}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{Experiments/Progress_Accuracy_model_stitch_4096-shot_train_and_test_final.png}
 \caption{ }
 \label{fig:Progress_Accuracy_model_stitch_4096-shot_train_and_test_final}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{Experiments/Progress_Model_Stitch_Agreement_Final_QNLI_4096.png}
 \caption{ Model Stitch Agreement Final QNLI 4096-shot }
 \label{fig:Progress_Model_Stitch_Agreement_Final_QNLI_4096}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.32\textwidth}
 \centering
 \includegraphics[width=\textwidth]{Experiments/Progress_Model_Stitch_Agreement_Diverge_QNLI_4096.png}
 \caption{ Model Stitch Agreement Diverge QNLI 4096-shot }
 \label{fig:Progress_Model_Stitch_Agreement_Diverge_QNLI_4096}
 \end{subfigure}
 \caption{}
 \label{fig:Stitch_update}
\end{figure}


==> ContinualLearning.tex <==

\iffalse
\section{Arithmetic}



\begin{table*}[!htbp]
\centering
%
\begin{tabular}{l|c|cc|c|c|c|c|} \toprule
 % \cellcolor[]{ggreen!15}
 Dataset & $\%$ Intersection &  Model & Purify &  \multicolumn{2}{c}{Stitch}  &  \multicolumn{2}{c}{Model / Stitch}  \\ 
 \midrule
 & & & & Direct & Intersect only & Non-stitch & Non-stitch + Intersect  \\
 \midrule
 & & (1.2, 1.3, 0.3) & & (0.8, 1.8, 0.2) &  (1.2, 2.0, 0.0) & (1.7, 1.9, 0.2)  &  ( 1.5, 2.0, 0.1 )  \\
 \midrule
 QNLI & & 83.8 & 81.91 & 77.17 & 60.77 &  81.53 & 82.39\\
 SST-2 & & 89.56 & 50.92 & 88.99 & 85.67  & 72.36 & 86.12\\
 ag news & & 88.75 & 77.72 & 77.27 & 88.63 & 88.38 & 88.71\\
 \midrule \midrule
 & & & & (0.2, 0.3, 0.7) & (0.3, 0.0, 0.0) & (0.6, 0.0, 0.7)  &  ( 1.2, 0.0, 1.1 )  \\
 \midrule
 QNLI & & 81.32 & & 59.02 & 64.77 & 77.99 & 80.41\\
 MNLI & & 71.82 & & 71.75 & 72.12 & 66.28 & 72.45\\
 SNLI & & 80.99 & & 80.36 & 77.40 & 80.97 & 83.82\\
 \bottomrule
\end{tabular}
\caption{Coexistence of models.}
\label{tab:roberta_coexistence}
\end{table*}





\begin{table*}[!htbp]
\centering
%
\begin{tabular}{l|c|c|c|c|} \toprule
 % \cellcolor[]{ggreen!15}
 Method & SST-2 & ag news & QNLI \\ 
 \midrule
 Train entire model & 92.63 (0.26) & 92.02 (0.43) & 86.88 (0.43) \\
 Project to $1\%$ dense stitch & 91.89 (0.45)  & 89.1   (0.71)  & 85.51 (0.57) \\
 Project to $0.1\%$ dense stitch & 92.37 (0.34) & 89.47 (0.65)  & 85.67 (0.45) \\
 Project to $0.01\%$ dense stitch & 92.04 (0.62) &  89.75  (0.37) & 84.41 (0.93) \\
 \bottomrule
\end{tabular}
\caption{Multitask.}
\label{tab:roberta_multitask}
\end{table*}
\fi




\begin{table*}[!htbp]
\centering
%
\begin{tabular}{l|c|c|c|c|c|} \toprule
 % \cellcolor[]{ggreen!15}
  & QNLI & ag news & SST-2 & QQP & SNLI \\ 
 \midrule
 QNLI & 86.84 &  71.7 (7.9) / 71.5 (3.9) & 76.3 (5.3) / 75.0 (3.9)  & 78.8 (2.2) / 75.9 (6.3)  &  70.3 (4.1) / 68.8 (0.6) \\
 ag news & & 93.1 & 89.5 (0.8) / 89.7 (1.0) & 87.2 (1.7) / 87.1 (3.7) & 85.4 (2.3) / 84.8 (3.0)   \\
 SST-2 & & & 92.0 & 89.3 (0.4) / 89.9 (0.7) & 86.3 (1.7) / 85.7 (2.2)  \\
 QQP & & & &  79.8 \\
 SNLI & & & & &  86.4 \\
 \bottomrule
\end{tabular}
\caption{Lifelong learning using stitch. Recall with 8 samples. Reported numbers: ( stitch parameters train / full model train ) across 5 subsets }
\label{tab:lifelong_learning_4shot}
\end{table*}



\begin{table*}[!htbp]
\centering
%
\begin{tabular}{l|c|c|c|c|c|} \toprule
 % \cellcolor[]{ggreen!15}
  & QNLI & ag news & SST-2 & QQP & SNLI  \\ 
 \midrule
 QNLI & 86.84 & 78.7 (2.4) / 77.3 (3.0)  & 78.4 (5.1) / 78.8 (2.4) & 81.1 (1.7) / 76.0 (7.0)  & 72.7 (3.1) / 68.7 (0.2)  \\
 ag news & & 93.1 & 91.3 (0.3)  / 91.4 (0.3) & 86.8 (3.7) / 87.1 (3.4) & 88.1 (1.6) / 85.6 (2.2) \\
 SST-2 & & & 92.0 & 90.3 (0.6) / 90.1 (0.9) & 87.5 (1.8) / 87.7 (1.5) \\
 QQP & & & & 79.8 \\
 SNLI & & & & &  86.4 \\
 \bottomrule
\end{tabular}
\caption{Lifelong learning using stitch. Recall with 16 samples. Reported numbers: ( stitch parameters train / full model train ) across 5 subsets}
\label{tab:lifelong_learning_8shot}
\end{table*}






\begin{table*}[!htbp]
\centering
%
\begin{tabular}{l|c|c|c|c|c|} \toprule
 % \cellcolor[]{ggreen!15}
  QNLI & ag news & SST-2 & QQP & SNLI \\ 
 \midrule
 86.84 &  68.97 (16.46) / 56.08 (5.02) & 67.99 (15.34) / 64.22 (7.44) & 70.68 (20.06) / 64.73 (19.36) & 70.42 (14.87) / 68.68 (7.01)  \\
 & 93.1 & 85.12 (2.39) / 88.17 (2.25) & 84.66 (2.43) / 79.35 (3.49) & 84.54 (2.56) / 73.29 (5.10)    \\
 & & 92.0 & 91.35 (0.81) / 84.04 (3.75) & 88.99 (1.47) / 75.11 (4.00)   \\
 & & &  79.8 & 73.17 (3.02) / 69.22 (1.57)\\
  & & & &  86.4 \\
 \bottomrule
\end{tabular}
\caption{Lifelong learning using stitch. HT with 8 samples. Reported numbers: ( stitch parameters HT / full model HT ) across 5 subsets }
\label{tab:lifelong_learning_HT4shot}
\end{table*}



\begin{table*}[!htbp]
\centering
%
\begin{tabular}{c|c|c|c|c|} \toprule
 % \cellcolor[]{ggreen!15}
  QNLI & ag news & SST-2 & QQP & SNLI  \\ 
 \midrule
 86.84 & 77.38 (6.94) / 63.41 (4.09) & 75.82 (7.74) / 71.99 (4.48) & 78.83 (6.28) / 75.00 (4.52) & 74.73 (10.99) / 72.73 (3.51) \\
  & 93.1 & 86.64 (2.06) / 89.09 (1.06) & 86.10 (2.00) / 80.31 (2.77) & 86.06 (1.81) / 76.91 (4.46) \\
  & & 92.0 & 91.19 (0.74) / 88.39 (0.83) & 90.02 (0.76) / 80.50 (3.37)  \\
  & & & 79.8 & 74.52 (1.91) / 71.75 (3.51)\\
  & & & &  86.4 \\
 \bottomrule
\end{tabular}
\caption{Lifelong learning using stitch. HT with 16 samples. Reported numbers: ( stitch parameters HT / full model HT ) across 5 subsets}
\label{tab:lifelong_learning_HT8shot}
\end{table*}










\iffalse
\begin{table*}[!htbp]
\centering
%
\begin{tabular}{l|c|c|c|c|c|c|c|c|} \toprule
 % \cellcolor[]{ggreen!15}
  & QNLI & ag news & SST-2 & QQP & SNLI  \\ 
 \midrule
 QNLI & 86.84 & 78.5 (3.2) / 74.2 (4.4)  & 83.3 (2.9) / 80.1 (3.1)  & 80.5 (3.6) / 81.0 (0.7) & 72.4 (3.8) / 71.6 (2.0) \\
 ag news & & 93.1 & \\
 SST-2 & & & 92.0 & & 88.2 (1.6) / 87.3 (2.8) \\
 QQP & & & &  79.8 \\
 SNLI & & & & &  86.4 \\
 \bottomrule
\end{tabular}
\caption{Lifelong learning using stitch. Recall with 32 samples}
\label{tab:lifelong_learning}
\end{table*}
\fi



==> table_fig/Bitfit_compare.tex <==



\begin{table}[!htbp]
\centering


%
\footnotesize
\begin{tabular}{l|cc|cc} \toprule
 % \cellcolor[]{ggreen!15}
  %Dataset  &  \\
  \midrule%& k=6000 \\
  & \multicolumn{2}{c|}{SST-2} & \multicolumn{2}{c}{QNLI} \\
 Alg. & Acc./F1 & ECE & Acc./F1 & ECE\\
 \midrule
 SGD &  91.9 {\tiny( 0.4 ) } & 7.38 {\tiny( 0.38 ) }    & 86.5 {\tiny( 0.2 ) } &  6.41 {\tiny( 0.99 ) }\\
 %SST-2 (patch) &  92.43 {\footnotesize( 0.09 ) } &  3.15 {\footnotesize( 0.40 ) } & / / \\
 Adam &  92.4 {\tiny( 0.6 ) }  & 6.72  {\tiny( 0.83 ) } & 87.8 {\tiny( 0.6 ) } & 8.1  {\tiny( 2.29 ) } \\
 %QQP (patch)  &  76.32 {\footnotesize( 0.36 ) } & 3.16 {\footnotesize( 0.51 ) } & -  \\
 \bottomrule
\end{tabular}
\caption{We report the performance and calibration loss of BitFit trained with AdamW and SGD. For comparison with the patch model, please refer to \cref{tab:roberta_stitchtrain}. The patch model gets lower calibration loss compared to BitFit while suffering a small drop in accuracy. }
\label{tab:bitfit}
\end{table}




==> table_fig/Retraining_performance.tex <==



\begin{table}[!t]
\centering
%
\caption{We check whether the learned patch forms a sub-network inside the model. To do so, we reset the FT model to the pretrained model and retrain only using the parameters in the patch. We observe that the learned patch can achieve similar test performance as the fully-trained FT model itself while having a high agreement with the patch model. We further show the retrained model has low calibration error.\vspace{0.1in}}
\label{tab:roberta_stitchtrain}
\footnotesize
%\scriptsize
\begin{tabular}{l|c|c|c|c} \toprule
 % \cellcolor[]{ggreen!15}
  %Dataset  &  \\
  \midrule%& k=6000 \\
 Dataset & Acc./F1 & ECE &  TV diff. & Agreement \\
 \midrule
 SST-2  &  92.2 {\tiny( 0.7 ) } &  3.92 {\tiny( 0.69 ) } & 0.244 {\tiny( 0.02 )} & 95.16 {\tiny( 1.01 )}\\
 %SST-2 (patch) &  92.43 {\footnotesize( 0.09 ) } &  3.15 {\footnotesize( 0.40 ) } & / / \\
 QNLI  &  87.4 {\tiny( 0.5 ) } & 2.03 {\tiny( 1.09 ) } & 0.202 {\tiny( 0.03 )} & 91 {\tiny( 1.25 )} \\
 %QNLI (patch) &  84.71 {\footnotesize( 0.61 ) } & 0.97 {\footnotesize( 0.33 ) } & / / \\
 AG News & 91.2 {\tiny( 0.1 ) }   & 0.96 {\tiny( 0.2 ) } & 0.11 {\tiny( 0.02 ) } & 95.73 {\tiny( 0.66 )}\\
 %AG News (patch) & 91.2 {\footnotesize( 0.1 ) }  & 91.09 {\footnotesize( 0.16 ) } & -  \\
 QQP  &  78.1 {\tiny( 0.7 ) }  &  4.28 {\tiny( 1.31 ) }  & 0.232 {\tiny( 0.06 ) } & 90 {\tiny( 1.05 )}\\
 %QQP (patch)  &  76.32 {\footnotesize( 0.36 ) } & 3.16 {\footnotesize( 0.51 ) } & -  \\
 \bottomrule
\end{tabular}
\end{table}

==> table_fig/roberta_patch_CLS.tex <==
\begin{table*}[!htbp]
\centering
\caption{Patching Performance at extreme sparsity ($\le 0.01\%$) for a model trained with a head on the [CLS] token.}
\label{tab:roberta_patch_single}
%
\begin{tabular}{l|cc|cc|cc|cc} \toprule
 % \cellcolor[]{ggreen!15}
  & \multicolumn{4}{c|}{k=64} &  \multicolumn{4}{c}{k=4096} \\
  \midrule%& k=6000 \\
      & \multicolumn{2}{c|}{FT} & \multicolumn{2}{c|}{Patch} & \multicolumn{2}{c|}{FT} & \multicolumn{2}{c}{Patch} \\
  \midrule%& k=6000 \\
 Dataset & Acc. & ECE & Acc. & ECE & Acc. & ECE & Acc. & ECE \\
 \midrule
 SST-2 {\footnotesize(acc)} &   88.7 {\footnotesize(1.8)} &  &  &  & 92.6 {\footnotesize(0.2)} &  &  &  \\
 QNLI {\footnotesize(acc)}  &  74.4 {\footnotesize(2.4)} &  & &  & 87.9 {\footnotesize(0.8)} &   & &  \\
 AG News {\footnotesize(acc)} & 87.2 {\footnotesize(0.7)}  &  &  &  & 92.3 {\footnotesize(0.5)} & &   & \\
 \bottomrule
\end{tabular}
\end{table*}
